Some New Results With k-set agreement

In this article, we investigate the solvability of $k$-set agreement among $n$ processes in distributed systems prone to different types of process failures. Specifically, we explore two scenarios: synchronous message-passing systems prone to up to $t$ Byzantine failures of processes. And asynchronous shared memory systems prone to up to $t$ crash failures of processes. Our goal is to address the gaps left by previous works\cite{SSS,AsynchKset} in these areas. For Byzantine failures case we consider systems with authentication where processes have unforgeable signatures. For synchronous message-passing systems, we present an authenticated algorithm that achieves $k$-set agreement in only two rounds, with no constraints on the number of faults $t$, with $k$ determined as $k \geq \lfloor \frac{n}{n-t} \rfloor + 1$. In fact the lower bound for $k$ is $k \geq \lfloor \frac{n}{n-t} \rfloor $ that is obtained by an algorithm based on traditional consensus with $t+1$ rounds. In asynchronous shared memory systems, we introduce an algorithm that accomplishes $k$-set agreement for values of $k$ greater than $ \lfloor \frac{n-t}{n-2t} \rfloor +1$. This algorithm uses a snapshot primitive to handle crash failures and enable effective set agreement.

==> contribution_o.tex <==
\section{\texorpdfstring{$k$-Set Agreement in an authenticated Message Passing Model}{}}
\label{sec:cont}

In this section, we explore set agreement in a message-passing model with authentication. Our focus is on ensuring reliable communication between processes through the exchange of \textbf{authenticated} messages in the TRB. Each received message is signed by the sender, guaranteeing its authenticity. Furthermore, we assume that the communication is reliable, meaning that messages are neither lost, forged, nor generated by the network.

Our objective is to present an authenticated algorithm that achieves $k$-set agreement in two rounds, with no constraints on the number of failures $t$. The value of $k$ is determined as $k = \lfloor \frac{n}{n-t} \rfloor + 1$. However, to achieve optimal agreement, we introduce an algorithm that spans $t+1$ rounds and guarantees $k$-set agreement for $k = \lfloor \frac{n}{n-t} \rfloor$ for any value of $t$. This algorithm leverages $n$ instances of the \textbf{Terminating Reliable Broadcast} (TRB), where the delivered value represents the proposed value for the set agreement. 




\subsection{A two round $k$-Set Agreement  in a  $\mathcal{BSMP}_{n,t}[Auth]$ Model}
We first present a two round algorithm, that ensures \emph{$k$SA} for $k= \lfloor \frac{n}{n-t} \rfloor +1$, this is an authenticated algorithm where the messages sent by processes are signed.  This prevents any faulty process from forging the signature of a correct process or misrepresenting the value sent by a correct process.



\subsection*{The Algorithm}

Algorithm \ref{2roundBSMP} ensures $k$-set agreement for $k= \lfloor \frac{n}{n-t} \rfloor + 1$ and $\forall t$. where the processes exchanges their messages in two rounds. A process $p_i$ in the first round send its initial value $v_i$, and receives every other process' initial value if any, it stores it an a vector $V_i$, and in the second round it sends it vector to every other process and receive from every $p_j$ a vector $V_j$ if any.




% Algorithm 

\begin{algorithm}[]
	
	\SetAlgoLined
	\KwIn{$v_i$  initial value}
	\KwResult{decide}
	
	\Comment{Local variables}  \label{phase1}
	$V_i$ Vector of decision of size $n$ initialized to $\perp$\\
		$M_i[i][i] = V_i[i] \leftarrow    v_i  $ \label{broadcast2round}; \\
{\bf for all} $k,\ell \neq i$ {\bf do} $M_i[j][k]\leftarrow \bot${\bf end for}; \\
	
	\BlankLine 
\Comment{----------------------- round 1  ----------------------------------------}

	\BlankLine
	Send the value $M_i[i][i]$ to all the processes ; \\
	\textbf{When} $p_i$ recevies $v_j$ from $p_j$ \textbf{do} $M_i[i][j] \leftarrow v_j$; \\ 

	\BlankLine
	\Comment{----------------------- round 2  ----------------------------------------}
	
	 Send  the vector  $V_i = M_i[i][*]$  to all the processes;\\
	
	\textbf{when } $p_i$ receives a vector $V$  from $p_j$ 
	\textbf{do}  $M_i[j]\leftarrow V$;         \\
	
		\Comment{-------------------  at the end of round 2  -----------------------------------}
\For{$j=1$ \KwTo $n$, with $j\neq i $ }
{   
	\For{$\ell,k =1$ \KwTo $n$, with $(\ell,k) \neq j $}
		{ 	\uIf{ $M_i[k][j] \neq M_i[\ell][j]$  }{  
				$V_i[j] = \perp$;
			} 
			\Else{
				$V_i[j]= v_j $; 
		} }
}


		\Comment{------------ Decision at the end of round 2  ---------------------}
	  \If{$p_i$ finds in $V_i$, $n-t$ values equal to $v_i$ }{  
		decide \textit{$v_i$;} \label{Dinit2round}
	} 
	\Else{
		decide $\perp$ \; \label{bottom2round}
	}
	
	
	
	
	
	
	\caption{Solving $k$-SA in $\mathcal{BSMP}_{n,t}[\forall t, Aut]$}
	\label{2roundBSMP}
\end{algorithm}


\subsection*{Proof of the algorithm}
Each process manages a local matrix  $M_i[1..n][1..n]$,  such that
$M_i[i][i]$ is initialized to the value proposed by $p_i$ and
all the other entries are initialized to $\bot$. 
In the first round each $p_i$ sends $M_i[i][i]$
to all the processes and assigns to  $M_i[i][j]$
the value it receives from $p_j$ .It is important to note that these sent messages are authenticated, ensuring that if $p_i$ receives a value $v_j$ from $p_j$, it can only come from $p_j$ and not from any other source.
Then at the second round, each process $p_i$ broadcasts its
$M_i[i][\ast]$ vector, and the received vectors from other processes
are used to update the matrix $M_i$ as follows: $p_i$ receives from
$p_j$ the vector $M$ that it stores it in $M_i[j] [\ast]$. An example of  $p_i$'s matrix $M_i$ is represented in Figure \ref{matrix mi}.  At the conclusion of this round, process $p_i$ compares the values of each column. If it detects that a process has sent two different values to two different processes, it sets its own values in $V_i$ to $\perp$. To guarantee the Validity property, if $p_i$ finds $n-t$ values in $V_i$ that are equal to its own initial value $v_i$, it decides on $v_i$ as the agreed value. Otherwise, it decides on $\perp$.

\begin{figure}[htb!]
	\centering
	\[M_i = 
	\begin{tikzpicture}[baseline=(math-axis),every right delimiter/.style={xshift=-3pt},every left delimiter/.style={xshift=3pt}, arrow/.style = {thick, -stealth}]%
		\matrix [matrix of math nodes,left delimiter=(,right delimiter=)] (matrix)
		{
			M_{11} && \cdots && M_{1i} && \cdots && M_{1j} && \cdots &&  M_{1n} \\
			\vdots &&        && \vdots &&        &&\vdots  \\
			|(Mi1)| M_{i1} && |(Mi2)| \cdots && |(Mi3)| M_{ii} = v_i && |(Mi4)| \cdots && |(Mi5)| M_{ij} && |(Mi6)| \cdots && |(Mi7)|  M_{in} \\
			\vdots &&        && \vdots &&        && \vdots  \\
			|(Mj1)| M_{j1} && |(Mj2)| \cdots && |(Mj3)| M_{ji} && |(Mj4)| \cdots && |(Mj5)| M_{jj} = v_j && |(Mj6)| \cdots && |(Mj7)|  M_{jn} \\
			\vdots &&        && \vdots &&        && \vdots  \\
			M_{n1} && \cdots && M_{ni} && \cdots && M_{nj} && \cdots &&  M_{nn} \\
		} ;
		\node (i)[color = red, draw,dashed,inner sep=0pt,fit=(Mi1) (Mi7)] {};
		\node (s1) at (4,2) {$M_i[i] [\ast]$};
		\draw [arrow, red] (s1) to (i);
		
		\node (j)[color = blue, draw,dashed,inner sep=0pt,fit=(Mj1) (Mj7)] {};
		\node (s2) at (4,-2) {$M_i[j] [\ast]$};
		\draw [arrow, blue] (s2) to (j);
		
		\coordinate (math-axis) at ($(matrix.center)+(0em,-0.25em)$);
		
	\end{tikzpicture}\]
	\caption{Matrix $M_i$}
	\label{matrix mi}
\end{figure}


\begin{lemma}
	Let $p_i$ be a correct process with matrix $M_i$, and let  $p_\ell$ and $p_j$ be two processes. If  $M_i[i][j] \neq M_i[\ell][j]$, which means that if process $p_j$ sent two distinct values to $p_i$ and $p_\ell$, then $p_j$ is Byzantine.
\end{lemma}
 
 \begin{proof} \label{byzproc}
 	By contradiction, lets suppose that $p_j$ is correct and send the same value to everyone, thanks to the authentication, $p_j$'s message cannot be forged or lied about, then all the processes in $\Pi$ will have the same view on $p_j$' value, and all the processes correct or Byzantine will relay the same message sent by $p_j$.
 	
 \end{proof}

\begin{lemma}
	[Validity] if all the correct processes propose the same value, they decide that value.
\end{lemma}

\begin{proof}
Consider a set $C$ consisting of correct processes that propose the value $v$. Since we have at most $t$ faulties, $C$ is consisting at least of $n-t$ correct processes. In order to satisfy the validity property, it is crucial that all correct processes decide on $v$. By the end of the second round, all correct processes will have at least $n-t$ values in their vector that are equal to $v$. Thus, in Line 17 of the algorithm, when a correct process observes this condition, it will decide on the value $v$.
\end{proof}


\begin{lemma}
	[Agrement] at most $\lfloor \frac{n}{n-t}\rfloor +1$ values are decided.
\end{lemma}

\begin{proof}
Let $e$ be any execution of the algorithm.
In $e$, there are  at most $t$ Byzantine failures. Let $ 0\le f\le t$
the actual number of Byzantine processes in $e$.

If a correct process $p$ decides a value $v$ different from $\bot$,
then there are  at least $n-f$ correct processes, including $p$,
that have this value as input.
%
Then at most  $\lfloor\frac{n}{n-f}\rfloor$  values are decided by correct processes in $e$.  The function {\small{$\lfloor \frac{n}{n-f}	\rfloor$}} of $f$ is growing, as $f\le t$ its maximum is for $f=t$, consequently at most  {$\lfloor \frac{n}{n-t}\rfloor $}
values different from $\bot$ are decided by correct processes in $e$. Moreover, $\bot$ may be decided. Then we have at most $\lfloor \frac{n}{n-t}\rfloor +1$  decided values.
\end{proof}

\begin{lemma}	
	[Termination] All the correct processes decide.
\end{lemma}

\begin{proof}
	All the correct processes will execute the two rounds, and decide at the end of the second round.
\end{proof}

By the above lemmas, we get the following theorem.

\begin{theorem} \label{th:2bsmp}
	Algorithm \ref{2roundBSMP}, ensures $\emph{$k$SA}$ in an authenticated message passing system with Byzantine failures for $k= \lfloor \frac{n}{n-t}\rfloor +1$
\end{theorem}



\subsection{An optimal $k$-Set Agreement in a  $\mathcal{BSMP}_{n,t}[Auth]$ Model} \label{sec:auth}
In this section, we present an algorithm that achieves optimality in terms of agreement. Specifically, we introduce an authenticated algorithm that ensures $k$-set agreement for $k = \lfloor \frac{n}{n-t} \rfloor$. To achieve this level of agreement, we are constrained to use more than two rounds. The algorithm incorporates a primitive that operates over $t+1$ rounds. Once again, there are no limitations on the number of failures $t$. This algorithm uses $n$ instances of the \textbf{Terminating Reliable Broadcast } (TRB), where the delivered value is the proposed value for the set agreement. 

For our algorithm, we will implement the authenticated TRB primitive for $n$ instances, where the $ith$ instance of TRB corresponds to the run instance where process $p_i$ is the sender in TRB.
%Definitions

\subsection*{The algorithm}

Algorithm \ref{BSMP}, ensures $k$-set agreement for $k= \lfloor \frac{n}{n-t} \rfloor$ and $\forall t$.
when $p_i$-$TRBroadcast(  v_i)$  is called then  process $p_i$ is the sender in the TRB algorithm, it stores its value in the vector $L_i$, while on the call of $q$-$deliver(m)$, a process $q$ is the sender in the TRB algorithm that sent a value $m$, and $q_i$ will deliver that value in the TRB algorithm.




% Algorithm 

\begin{algorithm}[]

\SetAlgoLined
\KwIn{$v_i$  initial value}
\KwResult{decide}

\Comment{Local variables}  

 $L_i $ is a $[1,\dots,n]$ vector initialized to $\perp$ \\
\BlankLine 
\Comment{Phase 1} 
\underline{On $p_i$-$TRBroadcast$ ($  v_i  $)} \\
\BlankLine
$L_i[p_i] \leftarrow    v_i  $ \label{broadcastBSMP} \\
\BlankLine
\underline{On $q$-$deliver(m)$:}\\
\BlankLine
$L_i[q] \leftarrow m$  \label{affectBSMP} \\

 \BlankLine
\Comment{Phase 2} 

  \uIf{$p_i$ finds in $L_i$, $n-t$ values equal to $v_i$ }{  
   decide \textit{$v_i$;} \label{DinitBSMP}
} 
  \uElseIf{$p_i$ finds a value $v$ repeated $n-t$}{decide $v$;}  \label{DecisionBSMP}
  \Else{
   decide $\perp$ \; \label{bottomBSMP}
 }
 



 \caption{Solving $k$-SA in $\mathcal{BSMP}_{n,t}[\forall t, Aut]$}
 \label{BSMP}
\end{algorithm}


%Proof of the Algorithm
\subsection*{Proof of the algorithm}
Every process $p$ holds a vector $L_i$ initialized to $\perp$. 	$n$ instances of $TRB$ are started, one per process, with each process being the sender in one instance. Every process p records in
vector $L_i$ the message $m$ delivered from process $q$. We consider $L_i$ the vector of the proposed values for the $k$-set Agreement. 
At the end of Phase 1, after each process sets its vector $L_i$, in order to ensure the Validity of the TRB, even if we have in the system Byzantine processes, all the vectors will be equal, and if all the correct processes propose the same value, we  will have at least $n-t$ values equal to their initial value. And to ensure the Validity of $k$-set agreement,  at the end of Phase 2, they will decide that value in Line \ref{DinitBSMP}. Now let's suppose we are in an execution where the correct processes do not have the same initial value, since we have at least $n-t$ correct processes, their initial value will be stored in $L$ due to the Validity of TRB, regarding the Byzantine, in order to have a common value among all the correct processes, the result stored in $L_i$ can be either $SF$ or an arbitrary value, but all the correct will have that same value in $L$, which leads to having the same vector $L$ at the end of Phase 1.
In order to ensure Agreement, all the correct processes decide by finding either $n-t$ values equal to their initial value, or any value repeated $n-t$ times, if not they will decide $\perp$.
We will see in the following lemma prove that if a process decides $\perp$, then no other correct process decides a value different from $\perp$.
%Les lemmas 

\begin{lemma}
   Let $p_i$ and $p_j$ be two correct processes that run Algorithm \ref{BSMP}, and we have $L_i = L_j$,  at the end of Phase 1. 
   \label{equalL}
\end{lemma}

\begin{proof}
From the  agreement of the TRB [\ref{agr-trb}], we have if a correct value delivers a value $m$, that value is delivered by all the correct processes, the delivered message is stored in the vectors of correct processes, then all the correct processes will have the same value in their vector.

\end{proof}

\begin{lemma}
The vector $L$ contains the initial value broadcast by correct processes.
\label{intivL}
\end{lemma}

 \begin{proof}
From the validity of the TRB [\ref{val-trb}],  if a value is broadcast  by a correct process, then this value is delivered by all the correct processes, since each process broadcasts its initial value, this value is delivered and then stored in $L$ (Line \ref{affectBSMP}).

 \end{proof}
 Hence, from the above Lemmas  we conclude that at the end of phase 1, all the correct processes have the same view on $L$.
\begin{lemma}
If a correct process $p_i$ decides a value $v$ different from $\perp$, no other correct process will decide $\perp$. 
\label{DecBottom}
\end{lemma}


\begin{proof}
    Let $p_i$ be a correct process that decides $v$ in Phase 2, then $p_i$ has found $n-t$ values equal to $v$, let $p_j$ be another correct process since the vector $L_i = L_j$ then $p_j$ should also find $|v| \ge n-t $. Thus every correct process will at least decide $v$.
    
\end{proof}

\begin{lemma}
    {\em [Validity]} If all the correct processes propose the same value,
  they decide this value.
  \label{lemVal}
\end{lemma}

\begin{proof}
Let $C$ be a set of correct processes that propose $v$, in order to ensure the Validity of the $k$-set agreement, from lemmas \ref{equalL} and \ref{intivL}  we have at least $n-t$ values equal to $v$, then in Line \ref{DinitBSMP}, all the correct processes will find that condition and decide $v$.
    
\end{proof}

 \begin{lemma}\label{simple:term}
{\em [Termination]} All the correct processes decide.

\end{lemma}

\begin{proof}
  All the correct processes will execute the two phases and will decide at the end of phase 2.
\end{proof}


\begin{lemma}\label{simple:agre}
{\em [Agreement]} At most $\lfloor \frac{n}{n-t} \rfloor $ values are decided by correct processes.

\end{lemma}

\begin{proof}
    From lemma \ref{equalL}, all the correct processes have the same value in $L$, we have to prove that all the correct processes will decide $\alpha$ values from $L$. 
    A decided value is repeated $n-t$ times in $L$, since $\alpha(n-t) \le n$ then $\alpha \le \lfloor \frac{n}{n-t} \rfloor $.
    
    \end{proof}
\begin{lemma}
   It is impossible to achieve $\lfloor \frac{n}{n-t} \rfloor -1 $ Set-Agreement.
    
\end{lemma}

\begin{proof}
    Let's suppose we organize the  $n$ processes into sets $C_i$ of size $n-t$ with $i = 1,\dots, \lfloor \frac{n}{n-t} \rfloor $
    Let's suppose we are in an execution where all the processes in the sets $C_i$ are correct and in each set $C_i$ the processes propose $v_i$, from lemma \ref{lemVal}, a process $p \in C_1$ will decide $v_1$. This execution is equivalent for $p$ to an execution where the processes of $C_1$ are correct and proposes $v_1$ and the processes of the other sets are Byzantine. In both executions in order to ensure validity $p$ should decide $v_1$. 
 If we do that for every set $C_i$, each set will decide a value and we will have $\lfloor \frac{n}{n-t} \rfloor $  decided value.
    
\end{proof}
By the above Lemmas, we get the following Theorem.

\begin{theorem} \label{th:bsmp}
When $n \le 2t$,  and $k=\lfloor \frac{n}{n-t}\rfloor$, 
Algorithm~{\em{\ref{BSMP}}} is optimal on the value $k$ of 
$k$-set agreement.
\end{theorem}





%proofs

% \begin{lemma}
%     If a correct process $p_i$  delivers $m$, then every other correct process will eventually deliver $m$.
% \end{lemma} 
% \begin{proof}
%     If $p_i$ decides $v$, either the general was correct and in order to ensure the Validity all the correct processes decide that value or the general is Byzantine, but since the messages are authenticated, the Byzantine is easily detected if it sends to different values to two correct processes if a  Byzantine process value is decided then all the correct process have that value and decide the same.
% \end{proof}



%Crash




